A new adaptive pricing framework for perpetual protocols using liquidity curves and on-chain oracles

This whitepaper introduces an innovative mechanism for pricing perpetual contracts and quoting fees to traders based on current market conditions. The approach employs liquidity curves and on-chain oracles to establish a new adaptive pricing framework that considers various factors, ensuring pricing stability and predictability. The framework utilizes parabolic and sigmoid functions to quote prices and fees, accounting for liquidity, active long and short positions, and utilization. This whitepaper provides a detailed explanation of how the adaptive pricing framework, in conjunction with liquidity curves, operates through mathematical modeling and compares it to existing solutions. Furthermore, we explore additional features that enhance the overall efficiency of the decentralized perpetual protocol.

==> charttest.tex <==


% Skew vs Dynamic Borrow Fee chart
\begin{figure}[htbp]
\centering
\begin{tikzpicture}
\begin{axis}[
    title={Skew vs Dynamic Borrow Fee},
    xlabel={Market Skew (\%)},
    ylabel={Dynamic Borrow Fee (\%)},
    xmin=0, xmax=100,
    ymin=0, ymax=500,
    xtick={0,20,40,60,80,100},
    ytick={0,100,200,300,400,500},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
]

\pgfplotstableread[col sep=comma]{dynamic.csv}\datatable

% Dynamic Borrow Fee (N=0.0125)
\addplot[
    color=blue,
    mark=square,
] table[x=Skew Percent V = (Skew/P)*100,y=Dynamic Borrow Fee (N=0.0125)] from \datatable;
\addlegendentry{Dynamic Borrow Fee (N=0.0125)}

% Dynamic Borrow Fee (N=0.0225)
\addplot[
    color=red,
    mark=triangle,
] table[x=Skew Percent V = (Skew/P)*100,y=Dynamic Borrow Fee (N=0.0225)] from \datatable;
\addlegendentry{Dynamic Borrow Fee (N=0.0225)}

% Dynamic Borrow Fee (N=0.0325)
\addplot[
    color=green,
    mark=o,
] table[x=Skew Percent V = (Skew/P)*100,y=Dynamic Borrow Fee (N=0.0325)] from \datatable;
\addlegendentry{Dynamic Borrow Fee (N=0.0325)}

\end{axis}
\end{tikzpicture}
\caption{Skew vs Dynamic Borrow Fee plot using different Dynamic Borrow Fee values.}
\label{fig:skew_vs_dynamic_borrow_fee}
\end{figure}

